A robust approach for estimating change-points in the mean of an AR(1) process

We consider the problem of multiple change-point estimation in the mean of a Gaussian AR(1) process. Taking into account the dependence structure does not allow us to use the dynamic programming algorithm, which is the only algorithm giving the optimal solution in the independent case. We propose a robust estimator of the autocorrelation parameter, which is consistent and satisfies a central limit theorem. Then, we propose to follow the classical inference approach, by plugging this estimator in the criteria used for change-points estimation. We show that the asymptotic properties of these estimators are the same as those of the classical estimators in the independent framework. The same plug-in approach is then used to approximate the modified BIC and choose the number of segments. This method is implemented in the R package AR1seg and is available from the Comprehensive R Archive Network (CRAN). This package is used in the simulation section in which we show that for finite sample sizes taking into account the dependence structure improves the statistical performance of the change-point estimators and of the selection criterion.

==> Abstract.tex <==
We consider the problem of multiple change-point estimation in the
mean of a Gaussian AR(1) process.  Taking into account the dependence
structure does not allow us to use the inference approach of the
independent case. Especially, the dynamic programming algorithm giving
the optimal solution in the independent case cannot be used
anymore. We propose a robust estimator of the autocorrelation
parameter, which is consistent and satisfies a central limit
theorem. Then, we propose to follow the classical inference approach,
by plugging this estimator in the criteria used for change-points
estimation. We show that the asymptotic properties of these estimators are the same as those of the classical estimators in the independent framework. The same plug-in approach is then used to approximate 
the modified BIC and choose the number of segments. Finally, we show, in the simulation section, that for finite sample size taking into account the dependence structure improves the statistical
performance of the change-point estimators and of the selection criterion.


==> ProofDeltaTCL.tex <==
\newcommand{\nstark}{{{n}^*_k}}
\newcommand{\nbark}{{\overline{n}_k}}
\newcommand{\deltastark}{{{\delta}^*_k}}
\newcommand{\deltabark}{{\overline{\delta}_k}}
\newcommand{\Wstark}{{{W}^*_k}}
\newcommand{\Wbark}{{\overline{W}_k}}
\newcommand{\Zstark}{{{Z}^*_k}}
\newcommand{\Zbark}{{\overline{Z}_k}}
\newcommand{\Istark}{{{I}^*_k}}
\newcommand{\Ibark}{{\overline{I}_k}}
\newcommand{\Ncal}{{\mathcal N}}

\paragraph{Proof of the TCL for $\deltabark$ under model \ref{bardet}.}
We denote
\begin{align*}
  \nbark & = \overline{t}_{k+1} - \overline{t}_k, 
  & 
  \nstark & = {t}^*_{k+1} - {t}^*_k,  
  &
  \Delta & = \rho^* - \overline{\rho}_n,
  \\
  \Wbark & = \sum_{\Ibark} w_i^*, 
  &
  \Wstark & = \sum_{\Istark} w_i^*,
  &
  \Zbark & = \sum_{\overline{I}_k} z_{i-1}, 
  &
  \Zstark & = \sum_{{I}^*_k} z_{i-1}.
\end{align*}
We want to prove that $\sqrt{\nbark}(\deltabark - \deltastark)$ is asymptotically Gaussian, where
$$
\deltabark = \nbark^{-1} (\Wbark - \Delta \Zbark).
$$
We have that $\sqrt{\nbark}(\deltabark - \deltastark)$
\begin{align*}
  = & {\nbark}^{-1/2} \left[\Wstark + \Delta \Zstark + (\Wbark - \Wstark) + \Delta (\Zbark - \Zstark) - \nbark \deltastark \right] \\
  = & \sqrt{\frac{\nstark}{\nbark}} 
  \left[
  \frac{\Wstark - \nstark \deltastark}{\sqrt{\nstark}} 
  + \Delta \frac{\Zstark}{\sqrt{\nstark}}  
  + \frac1{\sqrt{\nstark}} \sum_{i \in \Ibark \setminus \Istark} (w_i^* - \deltastark) 
  +  \frac{\Delta}{\sqrt{\nstark}} \sum_{i \in \Ibark \setminus \Istark} z_{i-1} 
  \right].
\end{align*}
We have that
\begin{enumerate}[($a$)]
 \item $\sqrt{{\nstark}/{\nbark}} \overset{P}{\rightarrow} 1$,
 \item $({\Wstark - \nstark \deltastark})/{\sqrt{\nstark}} \rightarrow \Ncal(0, \sigma^2)$,
 \item $\Delta \overset{P}{\rightarrow} 0$,
 \item ${\Zstark}/{\sqrt{\nstark}} \rightarrow \Ncal(0, \cdot)$,
 \item $\sum_{i \in \Ibark \setminus \Istark} (w_i^* - \deltastark) = O_P(1)$,
 \item $\sum_{i \in \Ibark \setminus \Istark} z_{i-1} = O_P(1)$.
\end{enumerate}
Applying Slutsky's Lemma to ($c$) and ($d$) gives $\Delta {\Zstark}/{\sqrt{\nstark}} \overset{P}{\rightarrow} 0$. Furthermore, because of ($e$) and ($f$) $(\sum_{i \in \Ibark \setminus \Istark} (w_i^* - \deltastark) +  {\Delta} \sum_{i \in \Ibark \setminus \Istark} z_{i-1})/\sqrt{\nstark}$ also converges to 0 in probability. Then, using Slustky again, the whole terms between square brackets is asymptotically distributed as $\Ncal(0, \sigma^2)$. The conclusion follows from ($a$). 

TO DO:
\begin{itemize}
\item Calculate $\sigma^2$
\item ($b$) via CLT
\item ($d$): find reference
\end{itemize}

\paragraph{Proof of the TCL for $\deltabark$ under model \ref{bardet}.}

